Generative Convolutional Networks for Latent Fingerprint Reconstruction

Performance of fingerprint recognition depends heavily on the extraction of minutiae points. Enhancement of the fingerprint ridge pattern is thus an essential pre-processing step that noticeably reduces false positive and negative detection rates. A particularly challenging setting is when the fingerprint images are corrupted or partially missing. In this work, we apply generative convolutional networks to denoise visible minutiae and predict the missing parts of the ridge pattern. The proposed enhancement approach is tested as a pre-processing step in combination with several standard feature extraction methods such as MINDTCT, followed by biometric comparison using MCC and BOZORTH3. We evaluate our method on several publicly available latent fingerprint datasets captured using different sensors.

==> figures/cmc_lumi_to_lumi.tex <==
% This file was created by matplotlib2tikz v0.5.7.
% The lastest updates can be retrieved from
% 
% https://github.com/nschloe/matplotlib2tikz
% 
% where you can also submit bug reports and leavecomments.
% 
\begin{tikzpicture}

\pgfplotsset{compat=newest} 

\definecolor{color0}{rgb}{1, 1, 1}

\tikzstyle{every node}=[font=\footnotesize]

\begin{axis}[
xlabel={Rank-N},
ylabel={Accuracy (\%)},
xmin=1, xmax=50,
ymin=0, ymax=30,
width=\figurewidth,
height=\figureheight,
at={(0\figurewidth,0\figureheight)},
xmajorgrids,
x grid style={lightgray},
ymajorgrids,
y grid style={lightgray},
axis line style={black},
axis background/.style={fill=color0},
legend style={at={(0.03,0.97)}, anchor=north west},%, draw=none, fill=color0},
legend cell align={left},
legend entries={{BFFT+MCC},{OUR+BFFT+MCC}}
]
\addplot [dashed, line width=0.75pt, red]
table {%
    1.0000    0
    50        30
};
\addplot [line width=1.25, red]
table {%
   50.0000   0
   1.0000    30
};
\end{axis}

\end{tikzpicture}
